How social media creators shape mass politics: A field experiment during the 2024 US elections

Political apathy and skepticism of traditional authorities are increasingly common, but social media creators (SMCs) capture the public's attention. Yet whether these seemingly-frivolous actors shape political attitudes and behaviors remains largely unknown. Our pre-registered field experiment encouraged Americans aged 18-45 to start following five progressive-minded SMCs on Instagram, TikTok, or YouTube between August and December 2024. We varied recommendations to follow SMCs producing predominantly-political (PP), predominantly-apolitical (PA), or entirely non-political (NP) content, and cross-randomized financial incentives to follow assigned SMCs. Beyond markedly increasing consumption of assigned SMCs' content, biweekly quiz-based incentives increased overall social media use by 10% and made participants more politically knowledgeable. These incentives to follow PP or PA SMCs led participants to adopt more liberal policy positions and grand narratives around election time, while PP SMCs more strongly shaped partisan evaluations and vote choice. PA SMCs were seen as more informative and trustworthy, generating larger effects per video concerning politics. Participants assigned to follow NP SMCs instead became more conservative, consistent with left-leaning participants using social media more when right-leaning content was ascendant. These effects exceed the impacts of traditional campaign outreach and partisan media, demonstrating the importance of SMCs as opinion leaders in the attention economy as well as trust- and volume-based mechanisms of political persuasion.

==> Tables/Tables_short/table_understand_intervention.tex <==
\textit{Panel A: differences relative to control condition} \\ Predominantly-apolitical SMCs (quiz)&   -0.111***   &   -0.119***   &       0.027   &       0.027   &      -0.019   &      -0.021   &    0.166***   &    0.162***   &    0.165***   &    0.160***   &       0.042   &       0.042   &       0.013   &       0.011   \\
                    &     (0.036)   &     (0.033)   &     (0.035)   &     (0.033)   &     (0.034)   &     (0.032)   &     (0.036)   &     (0.034)   &     (0.038)   &     (0.036)   &     (0.038)   &     (0.036)   &     (0.031)   &     (0.030)   \\
%p value            &       0.002   &       0.000   &       0.446   &       0.412   &       0.580   &       0.515   &       0.000   &       0.000   &       0.000   &       0.000   &       0.260   &       0.233   &       0.675   &       0.701   \\
Predominantly-apolitical SMCs (follow)&      -0.048   &      -0.048   &       0.009   &       0.009   &       0.000   &      -0.004   &    0.098***   &    0.098***   &     0.091**   &     0.085**   &       0.036   &       0.036   &      -0.027   &      -0.031   \\
                    &     (0.035)   &     (0.033)   &     (0.034)   &     (0.032)   &     (0.033)   &     (0.030)   &     (0.035)   &     (0.033)   &     (0.037)   &     (0.035)   &     (0.037)   &     (0.035)   &     (0.030)   &     (0.028)   \\
%p value            &       0.170   &       0.148   &       0.778   &       0.782   &       0.996   &       0.890   &       0.005   &       0.003   &       0.014   &       0.015   &       0.330   &       0.302   &       0.374   &       0.271   \\
Predominantly-apolitical SMCs (recommendation)&      -0.054   &     -0.060*   &      -0.006   &      -0.006   &      -0.012   &      -0.013   &       0.048   &       0.052   &     0.083**   &     0.081**   &       0.019   &       0.019   &       0.005   &       0.008   \\
                    &     (0.035)   &     (0.033)   &     (0.035)   &     (0.032)   &     (0.034)   &     (0.032)   &     (0.037)   &     (0.034)   &     (0.037)   &     (0.035)   &     (0.037)   &     (0.034)   &     (0.032)   &     (0.029)   \\
%p value            &       0.126   &       0.067   &       0.851   &       0.842   &       0.729   &       0.680   &       0.185   &       0.132   &       0.026   &       0.019   &       0.596   &       0.574   &       0.871   &       0.797   \\
Predominantly-political SMCs (quiz)&      0.061*   &      0.055*   &      -0.017   &      -0.016   &   -0.109***   &   -0.104***   &     0.074**   &     0.078**   &      0.061*   &      0.063*   &      -0.002   &      -0.002   &      -0.036   &      -0.034   \\
                    &     (0.032)   &     (0.029)   &     (0.033)   &     (0.031)   &     (0.030)   &     (0.028)   &     (0.035)   &     (0.033)   &     (0.036)   &     (0.034)   &     (0.036)   &     (0.034)   &     (0.028)   &     (0.026)   \\
%p value            &       0.053   &       0.063   &       0.609   &       0.615   &       0.000   &       0.000   &       0.036   &       0.018   &       0.094   &       0.061   &       0.953   &       0.950   &       0.199   &       0.199   \\
Predominantly-political SMCs (follow)&      -0.050   &      -0.051   &    -0.066**   &    -0.062**   &     -0.056*   &     -0.053*   &     0.074**   &     0.077**   &       0.043   &       0.048   &      -0.042   &      -0.042   &      -0.044   &      -0.042   \\
                    &     (0.035)   &     (0.032)   &     (0.033)   &     (0.031)   &     (0.032)   &     (0.030)   &     (0.036)   &     (0.034)   &     (0.036)   &     (0.034)   &     (0.036)   &     (0.034)   &     (0.028)   &     (0.027)   \\
%p value            &       0.152   &       0.110   &       0.046   &       0.045   &       0.075   &       0.072   &       0.039   &       0.021   &       0.244   &       0.157   &       0.240   &       0.213   &       0.120   &       0.118   \\
Predominantly-political SMCs (recommendation)&       0.006   &      -0.004   &       0.018   &       0.019   &      -0.027   &      -0.023   &     0.077**   &     0.082**   &       0.053   &       0.055   &     -0.068*   &    -0.068**   &     -0.051*   &     -0.048*   \\
                    &     (0.034)   &     (0.032)   &     (0.036)   &     (0.033)   &     (0.034)   &     (0.032)   &     (0.036)   &     (0.033)   &     (0.037)   &     (0.035)   &     (0.036)   &     (0.034)   &     (0.030)   &     (0.028)   \\
%p value            &       0.868   &       0.893   &       0.612   &       0.574   &       0.424   &       0.460   &       0.030   &       0.014   &       0.155   &       0.113   &       0.060   &       0.046   &       0.085   &       0.088   \\
Non-political SMCs (quiz)&   -0.206***   &   -0.210***   &     0.079**   &     0.075**   &      -0.035   &      -0.040   &    0.155***   &    0.152***   &    0.200***   &    0.192***   &    0.108***   &    0.108***   &      -0.023   &      -0.025   \\
                    &     (0.036)   &     (0.034)   &     (0.036)   &     (0.034)   &     (0.033)   &     (0.031)   &     (0.036)   &     (0.034)   &     (0.037)   &     (0.034)   &     (0.037)   &     (0.035)   &     (0.031)   &     (0.029)   \\
%p value            &       0.000   &       0.000   &       0.029   &       0.027   &       0.286   &       0.192   &       0.000   &       0.000   &       0.000   &       0.000   &       0.003   &       0.002   &       0.453   &       0.383   \\
Non-political SMCs (follow)&   -0.106***   &   -0.123***   &      -0.009   &      -0.010   &      -0.033   &      -0.033   &     0.072**   &     0.076**   &    0.115***   &    0.113***   &       0.010   &       0.010   &      -0.002   &       0.004   \\
                    &     (0.036)   &     (0.034)   &     (0.035)   &     (0.033)   &     (0.034)   &     (0.032)   &     (0.036)   &     (0.034)   &     (0.038)   &     (0.035)   &     (0.038)   &     (0.035)   &     (0.031)   &     (0.029)   \\
%p value            &       0.003   &       0.000   &       0.808   &       0.769   &       0.337   &       0.295   &       0.045   &       0.024   &       0.002   &       0.001   &       0.782   &       0.769   &       0.943   &       0.902   \\
Non-political SMCs (recommendation)&      -0.027   &      -0.039   &       0.013   &       0.015   &      -0.023   &      -0.019   &      0.064*   &      0.067*   &       0.049   &       0.054   &       0.018   &       0.018   &      -0.032   &      -0.022   \\
                    &     (0.035)   &     (0.033)   &     (0.036)   &     (0.034)   &     (0.035)   &     (0.032)   &     (0.037)   &     (0.035)   &     (0.038)   &     (0.035)   &     (0.039)   &     (0.036)   &     (0.030)   &     (0.028)   \\
%p value            &       0.440   &       0.229   &       0.710   &       0.655   &       0.501   &       0.548   &       0.079   &       0.054   &       0.198   &       0.130   &       0.634   &       0.614   &       0.296   &       0.443   \\
SMS/email message   &      -0.033   &      -0.036   &       0.033   &       0.035   &       0.003   &      -0.002   &       0.024   &       0.023   &      -0.006   &      -0.009   &     0.065**   &     0.065**   &      -0.030   &      -0.031   \\
                    &     (0.028)   &     (0.026)   &     (0.029)   &     (0.027)   &     (0.028)   &     (0.026)   &     (0.029)   &     (0.027)   &     (0.030)   &     (0.028)   &     (0.030)   &     (0.029)   &     (0.025)   &     (0.023)   \\
%p value            &       0.239   &       0.164   &       0.244   &       0.195   &       0.905   &       0.925   &       0.406   &       0.397   &       0.830   &       0.756   &       0.032   &       0.023   &       0.220   &       0.184   \\
\midrule \textit{Panel B: differences between treatment conditions} \\ PA SMCs (quiz) - NP SMCs (quiz)&     0.095**   &     0.091**   &      -0.052   &      -0.048   &       0.016   &       0.019   &       0.011   &       0.009   &      -0.035   &      -0.032   &      -0.066   &      -0.066   &       0.036   &       0.036   \\
                    &     (0.042)   &     (0.040)   &     (0.042)   &     (0.039)   &     (0.038)   &     (0.035)   &     (0.042)   &     (0.040)   &     (0.044)   &     (0.041)   &     (0.043)   &     (0.041)   &     (0.036)   &     (0.033)   \\
%p value            &       0.024   &       0.023   &       0.207   &       0.215   &       0.671   &       0.582   &       0.789   &       0.811   &       0.427   &       0.434   &       0.126   &       0.105   &       0.310   &       0.276   \\
PP SMCs (quiz) - NP SMCs (quiz)&    0.268***   &    0.265***   &    -0.096**   &    -0.091**   &    -0.074**   &    -0.064**   &     -0.080*   &     -0.074*   &   -0.139***   &   -0.129***   &   -0.110***   &   -0.110***   &      -0.013   &      -0.009   \\
                    &     (0.039)   &     (0.037)   &     (0.040)   &     (0.038)   &     (0.034)   &     (0.032)   &     (0.041)   &     (0.039)   &     (0.042)   &     (0.039)   &     (0.042)   &     (0.039)   &     (0.033)   &     (0.030)   \\
%p value            &       0.000   &       0.000   &       0.017   &       0.016   &       0.032   &       0.048   &       0.053   &       0.058   &       0.001   &       0.001   &       0.008   &       0.005   &       0.697   &       0.779   \\
PA SMCs (quiz) - PP SMCs (quiz)&   -0.172***   &   -0.174***   &       0.044   &       0.043   &     0.090**   &     0.084**   &     0.091**   &     0.084**   &     0.104**   &     0.097**   &       0.044   &       0.044   &       0.049   &       0.045   \\
                    &     (0.039)   &     (0.036)   &     (0.039)   &     (0.036)   &     (0.036)   &     (0.033)   &     (0.041)   &     (0.039)   &     (0.043)   &     (0.040)   &     (0.042)   &     (0.040)   &     (0.033)   &     (0.031)   \\
%p value            &       0.000   &       0.000   &       0.259   &       0.241   &       0.012   &       0.012   &       0.027   &       0.031   &       0.016   &       0.017   &       0.290   &       0.263   &       0.138   &       0.148   \\
PA SMCs (quiz) - SMS/email message&    -0.078**   &    -0.083**   &      -0.007   &      -0.008   &      -0.022   &      -0.018   &    0.142***   &    0.139***   &    0.171***   &    0.169***   &      -0.023   &      -0.023   &       0.044   &       0.042   \\
                    &     (0.036)   &     (0.033)   &     (0.035)   &     (0.033)   &     (0.034)   &     (0.031)   &     (0.036)   &     (0.034)   &     (0.038)   &     (0.036)   &     (0.038)   &     (0.036)   &     (0.031)   &     (0.029)   \\
%p value            &       0.031   &       0.013   &       0.845   &       0.806   &       0.511   &       0.562   &       0.000   &       0.000   &       0.000   &       0.000   &       0.545   &       0.521   &       0.154   &       0.141   \\
PP SMCs (quiz) - SMS/email message&    0.095***   &    0.091***   &      -0.050   &      -0.051   &   -0.112***   &   -0.102***   &       0.050   &      0.055*   &      0.067*   &     0.072**   &     -0.067*   &    -0.067**   &      -0.006   &      -0.003   \\
                    &     (0.032)   &     (0.029)   &     (0.033)   &     (0.031)   &     (0.030)   &     (0.028)   &     (0.035)   &     (0.033)   &     (0.036)   &     (0.034)   &     (0.036)   &     (0.034)   &     (0.027)   &     (0.025)   \\
%p value            &       0.003   &       0.002   &       0.130   &       0.106   &       0.000   &       0.000   &       0.152   &       0.095   &       0.062   &       0.033   &       0.060   &       0.047   &       0.836   &       0.909   \\
\midrule Observations&       3,525   &       3,525   &       3,525   &       3,525   &       3,525   &       3,525   &       3,525   &       3,525   &       3,525   &       3,525   &       3,525   &       3,525   &       3,525   &       3,525   \\
R$^2$               &        0.11   &        0.14   &        0.11   &        0.12   &        0.12   &        0.14   &        0.13   &        0.13   &        0.11   &        0.13   &        0.12   &        0.12   &        0.10   &        0.12   \\
Number of LASSO-selected covariates&               &           5   &               &           1   &               &           5   &               &           1   &               &           4   &               &           0   &               &           2   \\
Control outcome mean&        0.73   &        0.73   &        0.30   &        0.30   &        0.28   &        0.28   &        0.29   &        0.29   &        0.34   &        0.34   &        0.38   &        0.38   &        0.21   &        0.21   \\
Control outcome standard deviation&        0.44   &        0.44   &        0.46   &        0.46   &        0.45   &        0.45   &        0.45   &        0.45   &        0.47   &        0.47   &        0.49   &        0.49   &        0.41   &        0.41   \\
Outcome range

